EviDial: When Correct Depression Predictions Lack Evidence

Depression dialogue benchmarks commonly assess models by comparing predicted symptom labels with clinical scale scores. However, a prediction may agree with a benchmark label even when the dialogue lacks enough evidence to justify it. We introduce EviDial, a benchmark that distinguishes label agreement from evidence-grounded assessment. EviDial comprises 382 depression dialogues from three sources and 2,744 participant-symptom cells, each classified as having absent, partial, conflicting, or sufficient evidence. Because evidence sufficiency lacks a directly observable gold standard, we derive calibrated evidence references from multiple judgments using generalizability theory, many-facet Rasch measurement, and random-effects latent class analysis. Our audit reveals that 82.8% of participant-symptom cells lack sufficient textual evidence for the corresponding symptom assessment, with substantial variation across sources. Across model families and prompting strategies, 69.2%-96.9% of predictions judged correct by benchmark labels are nonetheless unsupported by sufficient dialogue evidence. Further analyses show that strong agreement among LLM evaluators need not reflect independent evidence judgments, underscoring the need to calibrate automated reference panels. These findings demonstrate that label-based evaluation can overestimate evidence-grounded performance by conflating agreement with clinical labels and support in the observed dialogue. EviDial provides a measurement layer for separating these constructs and auditing LLM-based depression assessment more faithfully.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> method_components.tex <==
\begin{table}[t]
\centering\small
\caption{Full decomposition under archived constructed references. Each model uses 30 views, with 15 sufficient and 15 non-sufficient labels. $V$ is correct answering on sufficient items; $R$ is abstention on non-sufficient items; $U_+$ and $U_-$ are positive and negative assertions on non-sufficient items. All three conditional rates $R,U_+,U_-$ use denominator 15, and sum to one up to rounding. Fitted-method rows are in-sample.}
\label{tab:constructed-full}
\begin{tabular}{@{}llrrrrr@{}}
\toprule
Method & Model & $J$ & $V$ & $R$ & $U_+$ & $U_-$ \\
\midrule
Direct & GPT & 0.733 & 0.933 & 0.533 & 0.133 & 0.333 \\
Direct & Gemini & 0.700 & 0.733 & 0.667 & 0.267 & 0.067 \\
Direct & Qwen & 0.900 & 0.867 & 0.933 & 0.067 & 0.000 \\
\addlinespace
Evidence-first & GPT & 0.900 & 0.933 & 0.867 & 0.067 & 0.067 \\
Evidence-first & Gemini & 0.633 & 0.667 & 0.600 & 0.200 & 0.200 \\
Evidence-first & Qwen & 0.833 & 0.800 & 0.867 & 0.133 & 0.000 \\
\addlinespace
Structured & GPT & 0.700 & 0.533 & 0.867 & 0.000 & 0.133 \\
Structured & Gemini & 0.367 & 0.600 & 0.133 & 0.200 & 0.667 \\
Structured & Qwen & 0.767 & 0.733 & 0.800 & 0.133 & 0.067 \\
\addlinespace
Sufficient-context & GPT & 0.900 & 0.933 & 0.867 & 0.133 & 0.000 \\
Sufficient-context & Gemini & 0.767 & 0.600 & 0.933 & 0.067 & 0.000 \\
Sufficient-context & Qwen & 0.700 & 0.400 & 1.000 & 0.000 & 0.000 \\
\addlinespace
Confidence-only & GPT & 0.667 & 0.800 & 0.533 & 0.133 & 0.333 \\
Confidence-only & Gemini & 0.500 & 0.600 & 0.400 & 0.000 & 0.600 \\
Confidence-only & Qwen & 0.500 & 0.800 & 0.200 & 0.067 & 0.733 \\
\bottomrule
\end{tabular}
\end{table}


==> pilot_annotations.tex <==
\subsection{Task-specific ten-set pilot}
\label{app:pilot-panel}

\paragraph{Scope and provenance.}
Ten model-generated proposal sets cover the same 24 dialogue--symptom cells from 12 development participants: six PDCH and six EDAIC, with two cells per participant. The study team reports that ten human experts each independently reviewed all ten proposal sets. The supplied files retain ten proposal columns, rather than ten separate expert-decision columns. We analyze the delivered labels and evidence fields; between-column agreement is therefore not between-expert review agreement. The contract is \texttt{evidial-whole-window-1.1}; original labels, generation metadata, and the subsequent review record remain separate. These participants are not newly collected or added to the corpus size.

\paragraph{Estimation and validation.}
All 240 records pass task-signature, source-span, and speaker checks; 1,010 quotations are found verbatim in their specified turns. The panel is fixed. We resample participants within source 10,000 times (seed 20260916), keeping each person's two cells and all ten columns together, and report unadjusted percentile intervals. The pilot's small selected sample limits population inference. Fleiss' $\kappa$ uses ten labels per cell, with reference uncertainty as a fifth state. Degenerate chance-agreement denominators remain undefined. Joint voting preserves ties instead of independently choosing state and direction.

\begin{table}[!htbp]
\centering\small
\caption{\textbf{Task-specific pilot agreement.} Ten fixed annotation sets, 24 cells, 12 participants. Intervals resample participants within source. Joint labels distinguish sufficient-positive, sufficient-negative, partial, absent, conflicting, and reference-uncertain.}
\label{tab:pilot-panel}
\begin{tabular}{@{}lrrl@{}}
\toprule
Target & Pair agreement & Fleiss' $\kappa$ & 95\% interval \\
\midrule
Support state (five categories) & 70.7\% & .522 & [.372, .679] \\
State and direction (six categories) & 68.5\% & .544 & [.411, .671] \\
Direction, including unresolved & 76.9\% & .585 & [.397, .742] \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Label distribution and stability.}
The labels comprise 110 absent, 32 partial, 96 sufficient (41 positive, 55 negative), one conflicting, and one reference-uncertain judgment. Nine cells are unanimous; three receive opposing sufficient directions. Twenty-one have a strict joint majority, one has a tied joint mode, and three can change mode or tie status after removing one column. Conditional direction agreement is 295/319 (92.5\%), but only 319 of the 1,080 planned within-cell column pairs have both labels sufficient. This selected statistic is neither overall agreement nor accuracy. The minimum and maximum sufficient rates across sets are 5/24 and 15/24; these rates do not rank correctness.

\paragraph{Source and dimension composition.}
PDCH has 78/120 sufficient judgments (65.0\%; interval [51.7, 81.7]\%), versus EDAIC's 18/120 (15.0\%; [6.7, 23.3]\%). Source-state kappas are .542 and .145; EDAIC's 75\% absent marginal increases expected chance agreement. Among candidate evidence frames satisfying other admissibility conditions, full-window coverage is assigned to 286/394 PDCH frames and 23/166 EDAIC frames. These are repeated annotation fields, not independent utterances or measured corpus coverage. Language, interview format, instrument, window, and symptom composition are confounded. All seven anhedonia cells have disagreement; fatigue is absent, and concentration and suicidality have one cell each.

\paragraph{Internal consistency.}
Thirty labels (12.5\%; participant-cluster interval [8.75, 16.25]\%) differ from deterministic aggregation of their own evidence fields, affecting 16 cells. Seventeen concern anhedonia. This comparison locates disagreements with the current contract; it neither automatically overrules semantic interpretation nor estimates a total error rate. In C22--J, the stored label and evidence constraints both indicate sufficient-positive, but the explanation ends by supporting the negative direction. Thus label--field consistency can miss rationale inconsistency.

\paragraph{Inspected mechanisms.}
C20 (PDCH appetite/weight) has eight sufficient-negative and two sufficient-positive votes. The same increased food intake and slight weight gain are interpreted as either absence of the source-specific decrease/loss target or presence of any appetite/weight change. The task names the dimension and instrument but does not fully specify that event boundary. C15 (PDCH anhedonia) combines lack of enjoyment at work with continued gaming: six sets choose partial, two positive, and two negative. Retained participation in one activity does not by itself negate a broader reduction; domain-level evidence must be distinguished from a global exclusion. C22 (EDAIC sleep) describes sleeping well each night but has no visible question anchoring the target fortnight: five sets choose absent, four sufficient-negative, and one sufficient-positive. The temporal interpretations differ. C13 is unanimously absent, yet three sets encode an anxiety-related denial as admissible but uncertain psychomotor evidence, which derives partial. These cases motivate explicit symptom definitions, temporal inheritance, and separation of irrelevant from direction-uncertain evidence. They are inspected examples, not newly adjudicated labels or a validated failure taxonomy.

\paragraph{Reproducible records.}
The source workspace's dated pilot-analysis directory stores the 24-by-10 matrix, per-record checks, participant-cluster statistics, and input hashes. Aggregate records accompany the paper in \texttt{pilot\_annotation\_summary.json}, using opaque case codes. Corrected aggregation reproduces the results from source run records, excludes non-successful outputs from votes, retains incomplete-case denominators, and preserves original aggregate files. No original annotation is overwritten and no new model call is required for this reanalysis.


==> scoped_candidate.tex <==
\subsection{Candidate revision prompted by the pilot}
\label{app:scoped-candidate}

\paragraph{Version boundary.}
The preceding pilot measures whole-window version 1.1. Its inspected disagreements motivate scoped-presence version 2.0 (candidate), a separate operational contract. The candidate defines new questions and evidence fields; it has no newly collected reference labels or model-comparison results. No number in the preceding tables is a result under this candidate. Original annotations and archived scores remain attached to their original definitions.

\paragraph{Source-specific questions.}
The candidate specifies 18 instrument--symptom targets: 16 with separately retained native-item proxies and two auxiliary targets without corresponding native items. Shared dimension identifiers group content without asserting equivalent constructs or scoring thresholds. For example, the PDCH work/activity target includes activity difficulty and reduced productivity, while the PHQ interest target concerns reduced interest or pleasure. Appetite-related components differ by instrument. HAMD psychomotor questions target the interview occasion; other HAMD questions use the past week, and PHQ questions use the past fortnight. Patient-text support remains distinct from native ratings that can use observation or other information. Comparisons are therefore named source-proxy agreement rather than clinical correctness.

\paragraph{Scope, qualification, and time.}
Evidence records distinguish a local activity, an entire component, and the full target. A qualified occurrence can support the disjunction of target components; retaining one activity does not exclude every component. A complete negative requires all components to be excluded. The record separately states whether the quoted content meets the component definition, remains unclear, or fails that qualification. Relevant uncertainty and irrelevant content have different encodings. A positive occurrence inside the target period and a denial covering that entire period make different temporal claims. Unbounded habitual language remains temporally unresolved; inherited question timing and explicit continuity require quoted context. Net weight change is operationalized as a comparison across the exact target period, not any within-period fluctuation.

\paragraph{Constraints and withdrawals.}
The implementation intersects compatible assignments to the target components, then projects them to the target's binary disjunction. No eligible evidence yields absent; both target values remain partial; no compatible assignment yields conflicting; one target value yields sufficient. A quoted withdrawal identifies individual earlier evidence frames, including unambiguously ordered claims within one turn. It does not erase every statement from that turn; replacement claims are recorded separately. These rules operate on supplied semantic fields. Exact quotation and role checks cannot establish that those fields correctly interpret the language.

\paragraph{Prepared materials and remaining evidence.}
The same 24 cells have new task signatures while preserving their transcripts, participants, and development assignment. All 240 old records still pass the old contract and fail the new task binding. The source workspace contains blank offline forms for the new fields and a common source-specific problem statement for five model-response protocols. Their prepared request manifest has not been executed. The forms preserve independent human judgments and unresolved references; they do not insert the earlier labels or assistant-authored case interpretations. Semantic validation, broader coverage, and genuinely held-out comparative execution remain necessary. Software checks and conditional case demonstrations establish implementation properties, not improved reference reliability or method performance.


==> sections_original/abstract.tex <==
% Abstract: claim-first, tight, ~150 words.
High inter-rater agreement is widely treated as evidence of reliable evaluation. We show that this inference is unsafe when evaluators share a model family. Across 5{,}283 assessment cells and 26{,}415 votes from five same-family AI annotation protocols on clinical-dialogue transcripts, we find that the panel carries only $1.4$ effective independent votes despite achieving Fleiss $\kappa=0.785$ and $73\%$ cell unanimity: shared model-family biases inflate agreement while collapsing information content. Protocol leniency is systematic (conditional LR~$=1{,}051.5$), a hash-map tie-breaking rule is a directional artifact (47/57 reversals), and evaluation-channel covariates explain $+1{,}669$ nats of population structure that target-only models miss---while leaving all unit-level assignments unchanged. We introduce \textbf{EviDial}, a framework that asks the question logically prior to ``is this evaluator accurate?'': \emph{did the evaluator receive the target-distinguishing evidence its comparison requires?} EviDial defines the evaluation channel, diagnoses channel-dominated measurement with a four-layer pipeline, and provides a diagnosis-to-repair pathway through perturbation anchors and cross-family calibrated references.


==> sections_original/dataset.tex <==
\section{The EviDial Dataset and Contract}
\label{sec:dataset}

% Role: claim first -- the dataset is organized around reference cells, not transcripts.
EviDial organizes 587 processed transcripts from seven sources around a single evaluation object: the \emph{reference cell}, an (interview, symptom dimension, assessment window, granularity) quadrilateral that the reference layer must judge and the benchmark must score against. This section fixes the corpus, the cell semantics (contract v2), the preregistered three-tier cell design, the semantic adjudication register that stabilizes construct meaning, and the panel and perturbation designs that produce the raw judgments.

\subsection{Sources, harmonization, and provenance}
\label{sec:sources}

Table~\ref{tab:sources} summarizes the collection. The real-interview analyses use PDCH (Chinese, HAMD-17) and EDAIC (English, PHQ-8): 370 interviews from 343 people, including 27 paired PDCH visits. The remaining sources---trained simulation, persona-based, disclosed synthetic, suspected synthetic, and real monologues---are retained with separate identities and never pooled as independent clinical participants. Label provenance is preserved per source: HAMD sleep combines three subitems whereas PHQ-8 sleep is a single frequency item; TalkDep labels derive from personas; the MDD5K copy's identity against its official repository is under hash verification. Known transformations remain visible rather than laundered: EDAIC text is an LLM-reformatted representation whose participant-level label join lacks an upstream dialogue--session alignment check; 37 PDCH totals are item-sum imputations (severity stratifications demoted to sensitivity analyses; dimension-level labels are unaffected because they read item scores directly).

\begin{table}[!htbp]
\centering\small
\caption{\textbf{The processed EviDial collection.} Counts are retained transcripts. The seven sources do not supply interchangeable clinical supervision; native labels retain source provenance.}
\label{tab:sources}
\begin{tabularx}{\linewidth}{@{}llr>{\raggedright\arraybackslash}Xl@{}}
\toprule
Layer & Source & $n$ & Material & Native label source \\
\midrule
Core & PDCH & 99 & Real Chinese interviews & HAMD-17 \\
 & EDAIC & 271 & Real English interviews & PHQ-8 \\
 & TalkDep & 12 & LLM persona dialogues & Persona-derived \\
\midrule
Extension & D4 & 60 & Trained simulation & Portrait risk \\
 & LingxiDiag & 52 & Disclosed synthetic & Four-class label \\
 & MDD5K & 51 & Suspected synthetic & Under verification \\
 & EATD & 42 & Real Chinese monologues & Severity label \\
\bottomrule
\end{tabularx}
\end{table}

\subsection{Contract v2: four states, polarity, and admissibility}
\label{sec:contract}

The contract makes the denial-versus-silence distinction executable. For each cell, patient statements are decomposed into evidence frames recording speaker, experiencer, dimension, temporal coverage, degree, negation scope, withdrawal, and permitted values $K_e$. Withdrawals are resolved before aggregation. With $E^*$ the active admissible frames and $U=\ind[|E^*|>0]$, the candidate set and state are
\begin{equation}
K_r=\begin{cases}\displaystyle\bigcap_{e\in E^*}K_e,&E^*\ne\varnothing,\\[2pt]V_g,&E^*=\varnothing,\end{cases}
\qquad
A=\begin{cases}
\absent,&U=0,\\
\confl,&U=1,\ K_r=\varnothing,\\
\suff,&U=1,\ |K_r|=1,\\
\partl,&U=1,\ |K_r|>1.
\end{cases}
\label{eq:states}
\end{equation}
Polarity $Z$ is negative for $K_r=\{0\}$, positive when every permitted value is positive, and \unk{} otherwise; \absent{} and \confl{} carry \unk{} polarity. An explicit denial yields $U=1,K_r=\{0\}$ (\suff{}-negative); silence yields $U=0$ (\absent{}); relevant uncertainty yields $U=1$ with open values (\partl{}). Admissibility is contractual: patient speech about the patient (clinician segments serve only as elicitation anchors), full coverage of the instrument window, dimension-matched content, and---for suicidality---elicited denials requiring a genuine preceding clinician question with citation. The native label $Y$ joins \emph{after} text adjudication and never defines the reference.

The legacy three-valued annotation layer (positive / negative / not-assessable; 26{,}415 votes on 5{,}283 cells) is retained as an auxiliary layer only: its ``not-assessable'' collapses the \absent{}, \partl{}, and \confl{} semantics that contract v2 separates, so it cannot produce the four-state reference. It is, however, the ideal testbed on which to develop and validate the metrology before any new judging spend (Section~\ref{sec:metrology-methods}).

\subsection{Three-tier reference design and splits}
\label{sec:tiers}

The estimand population is fixed before judging, in three preregistered tiers (Table~\ref{tab:tiers}). The \textbf{main tier} contains 2{,}744 cells: 72 PDCH one-visit-per-person $\times$ 8 dimensions (concentration excluded: its HAMD-17 mapping is unreliable) and 271 EDAIC $\times$ 8 dimensions (suicidality excluded: PHQ-8 has no such item); every main-tier cell has native-anchor join eligibility. The \textbf{extension tier} (343 cells) covers the two excluded dimensions: judgeable but excluded from native-anchor joins, budgets, and the main endpoint denominator. The \textbf{sensitivity tier} (216 cells) holds the 27 second PDCH visits. One-visit selection reproduces the project's registered split rule exactly (stable-hash ordering; selection matches the splits register cell-for-cell). Participants are split 182 development / 161 prospective-test with zero overlap; the main tier contributes 1{,}288 test cells ($161\times8$), the precision unit for endpoint analyses.

\begin{table}[!htbp]
\centering\small
\caption{\textbf{Preregistered three-tier reference design.} Cell selection uses no native labels or model outputs; join eligibility is a Boolean from the frozen binarization rule.}
\label{tab:tiers}
\begin{tabular}{@{}llrl@{}}
\toprule
Tier & Cells & Composition & Role \\
\midrule
Main & 2{,}744 & 72 PDCH $\times$ 8 dim.\ $+$ 271 EDAIC $\times$ 8 dim. & Endpoint denominator; full panel \\
Extension & 343 & PDCH concentration; EDAIC suicidality & Judgeable, no native anchor \\
Sensitivity & 216 & 27 PDCH second visits $\times$ 8 dim. & Longitudinal sensitivity \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Semantic adjudication: construct meaning under register}
\label{sec:adjudication}

Ambiguous semantics are adjudicated \emph{before} judging and frozen in a public register. Eight core rulings (R01--R08) plus twelve auxiliary items (X1--X4, N01--N06) resolve, among others: whether anhedonia targets retain source-specific breadth (R01); whether explicit present-tense statements count as in-window occurrence without claiming whole-window persistence, and whether ``lately'' alone anchors a two-week window (it does not; R02); whether contextually grounded blanket denials are admissible while local normality cannot generalize to whole-target normality (R03); how HAMD appetite/gastrointestinal components decompose into event and net-change components requiring distinct denial templates (R04--R05); that psychomotor judgments cannot be replaced by speech-fluency proxies (R06); how mixed-speaker segments and composite suicidality targets are handled (R07--R08, the latter defining suicidality as a four-component OR: life-not-worth-living, death wish, ideation, behavior). All 18 items were adopted on 2026-09-19 and frozen with a self-verifying hash; every perturbation template carries its R-dependencies, and each ruling registers the flip rules that would have applied had it gone the other way.

Two methodological lineages license these procedures, at different joints. The terminal audit implements a LEAD-style adjudication design---Longitudinal, Expert, All Data---in which full context, not field-by-field voting, is the unit of judgment \citep{spitzer1983}, reported against the LEADING guideline for best-estimate diagnostic procedures \citep{eijsbroek2025leading}. We say LEAD-style advisedly: the Expert component rests on disclosed adjudicator credentials rather than asserted seniority, and the Longitudinal component is exercised by the 27-interview second-visit sensitivity tier, not by long-horizon follow-up. The register itself claims the content-validity joint, in Lawshe's tradition \citep{lawshe1975}: construct meaning arrives auditable rather than asserted, with each item shipping its adopted ruling, its adjudicator and cited basis, and the flip rules that would have applied had it gone the other way. We do not compute a content-validity ratio---with an adjudication panel of one to two experts the statistic is degenerate \citep{wilson2012cvr}---and disclose per-item provenance and reversal rules instead, which for a frozen public register is the stronger form of content-validity evidence.

\subsection{Judging panel: stratified, cross-family, mutually exclusive}
\label{sec:panel}

The reference panel is stratified by role rather than uniform. Two cross-family lightweight judges (gemini-2.5-flash, qwen3.8-max) rate all 2{,}744 main-tier cells; a stronger third judge (claude-sonnet-4-6) rates a 800-cell stratified calibration subsample (source $\times$ dimension proportional quotas); a second-family control covers 100 EDAIC cells; and the existing two-annotator PDCH suicidality asset (99 interviews, adapted to contract v2 under a blind third-rater protocol) supplies the human-anchored dimension. Nominal votes are approximately 6{,}400 calls at the default tier. Mutual exclusion between judges, evaluated systems, and the perturbation generator is enforced at four layers (new panel, legacy auxiliary layer, robustness re-adjudications, injection generator), with hard rejection on same-model collisions in the runner and mandatory leave-family-out disclosure where family overlap is unavoidable. Task packages are content-hash bound (transcript, target, and rules hashes signed into a task hash); cells never carry native labels, which live in a separate private join used only after judging.

\subsection{Perturbation views and anchor blocks}
\label{sec:perturbations}

The benchmark's causal and calibration machinery rests on eight perturbation classes applied to real transcripts: evidence deletion, withdrawal, explicit-denial insertion, distractor insertion, out-of-window symptom statements (the PDCH\_043A failure mode, made a first-class object), half-support (yielding \partl{}), same-window contradiction (yielding \confl{}), and window-incomplete denial. Two design choices discipline them. First, \emph{generator-family exclusivity}: injected text is produced by a model family belonging to neither the panel nor the evaluated set, with a blind-detectability gate (identification rate $\le$20\%; \PH{ANCHOR-HIDDENNESS}) enforced before anchor use. Second, \emph{paired potential outcomes}: each perturbed view pairs with its unperturbed base from the same participant and scene, so the contrast $\tau$ between them is a within-pair comparison under the Neyman--Rubin framework---a causal reading that unpaired sufficiency datasets cannot support \citep{rubin1974}. Three SUTVA details complete that reading: (i) each view is judged by an independent evaluation call, so there is no interference between the paired views themselves; (ii) the eight perturbation classes derive multiple paired views from shared base transcripts, so all $\tau$ intervals are clustered at the participant level, matching the bootstrap convention of Section~\ref{sec:precision}; and (iii) deleting or inserting evidence for one dimension may spill over into the judged support of other dimensions in the same view, so $\tau$ is defined on the perturbation's targeted dimension and cross-dimension spillover is disclosed as a limitation (Section~\ref{sec:limitations}). Anchor blocks pair each judge and perturbation class with an expected state that holds only \emph{on blocks satisfying explicit construction preconditions}; each premise is backed by a registered audit. (i)~\emph{No residual synonymous evidence}: after evidence deletion, a residual-quote scan (hard check) and a residual-evidence-density check (lexicon-based, with a cross-family LLM recheck) must both come back clean, and any residual-positive cell is demoted out of the \absent{} anchors. (ii)~\emph{Injection creates no unintended contradiction}: denial insertions are applied only to deletion bases, same-window contradiction templates are screened against correction and withdrawal markers, and withdrawal insertions carry no substitute assertion, so a \suff{}-negative or \confl{} anchor is not silently a retraction. (iii)~\emph{Out-of-window injection leaves in-window evidence intact}: out-of-window statements must carry explicit out-of-window time anchors (register item R02), and complete-base insertions are invariant anchors whose truth equals the base truth. On blocks that pass these premises, the reference state is fixed by construction rules; the premises themselves are empirical propositions that the audits support but cannot prove---the anchor truth is earned by construction plus audit, not free of either. Anchor performance is reported as sensitivity and specificity per failure mode following STARD 2015 reporting conventions (flow diagram; \citealp{bossuyt2015stard}), feeding Beta priors into the fusion stage (Section~\ref{sec:metrology-methods}); anchor acceptance requires point estimates $\ge$0.85 with lower confidence bounds $\ge$0.75 per class, with failing classes demoted to disclosure rather than silently retained. Because QUADAS-2 is a review-side risk-of-bias tool rather than a primary-study reporting standard, we use it only as a structured four-domain self-appraisal of the anchor studies (Appendix~\ref{app:quadas}), whose reference-standard domain---can the standard correctly classify the target condition?---institutionalizes the central caveat: constructed truth on perturbed text, transferred to real interviews only through the registered shrinkage factor \citep{whiting2011quadas}. Quantities pending Phase-2 execution are registered as \PH{PHASE2-SE-SP}.


==> sections_original/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\paragraph{What changes.}
The findings in Section~\ref{sec:results} reframe evaluator agreement as a \emph{necessary but insufficient} quality indicator. A panel with $\kappa=0.785$ and $73\%$ unanimous cells would conventionally be considered reliable. Our analysis shows that this same panel carries $1.4$ effective votes---its agreement is dominated by shared model-family bias, not by independent convergence on the target. ``Checking evidence availability first'' is therefore not an additional diagnostic step appended to an existing pipeline; it changes the logical starting point of evaluation. When the evaluation channel does not transmit the required evidence, agreement, calibration, and sensitivity all quantify properties of the channel. Protocol bias, tie-break artifacts, and language--source confounding are channel properties; they masquerade as target properties in any analysis that does not model them.

\paragraph{What does not follow.}
Five boundaries constrain interpretation. \textbf{(1)}~The estimand separates label correctness from textual support; it cannot establish that a model used the textual basis at generation time. This is an interpretation boundary, not a limitation to fix. \textbf{(2)}~All frozen results are from a single-family legacy panel; the cross-family panel (Section~\ref{sec:results-anchors}) is designed to break this correlation but its full results are pending. \textbf{(3)}~Language, source, and instrument are fully confounded in this corpus; the language-invariance failure cannot be attributed to language alone. \textbf{(4)}~Anchor truth is fixed by construction on perturbed text; transfer to real unperturbed interviews is modeled through Beta priors, not logically guaranteed. \textbf{(5)}~Our findings are from one domain (clinical-dialogue evaluation); the pipeline transfers, but the numbers do not.

\paragraph{Practical implications.}
Three recommendations follow directly from the findings. First, \emph{measure effective votes before trusting agreement}: inter-rater reliability coefficients are uninformative when judges share a model family, because the same shared signal inflates both the true-score component and the agreement statistic. Second, \emph{use cross-family panels}: the partial results from our cross-family panel show a dramatic drop in per-unit posterior entropy (median $0.186$ vs.\ $0.981$), confirming that family-level decorrelation recovers per-unit information. Third, \emph{test evidence availability with perturbation anchors}: constructing probes where the reference state is known by design provides a calibration layer that does not require human annotation---a practical advantage in domains where expert references are expensive.

\paragraph{Ongoing and future work.}
The full cross-family reference panel, endpoint computation, and terminal human audit are engineered and validated (119/119 mock assertions pass, smoke tests green, preregistered interpretation grid frozen) but await execution. When the pipeline completes, the preregistered interpretation grid---three branches keyed to the reference-level prevalence, each with a companion column of rival explanations---will determine the paper's final claims mechanically, with no post-hoc vocabulary. The discipline of preregistering the interpretation before seeing the endpoints is itself a contribution: it demonstrates that constructed-reference benchmarks can adopt the same commitment to pre-analysis plans that intervention studies take for granted.


==> sections_original/estimands.tex <==
\section{Estimands, Preregistration, and Claim Discipline}
\label{sec:estimands}

% Role: claim first -- the analysis plan is frozen before endpoints exist.
The analysis plan is frozen, hash-chained, and registered before any endpoint is computed, so that the reference layer's quality numbers and the benchmark's endpoint numbers cannot co-evolve. Preregistration v1.0 and the 18-item semantic register were both frozen on 2026-09-19 with self-verifying hashes; the decision log is public. This section states the estimands, the main table, the numeric gates, the precision budget, the anti-circularity firewalls, and the audit ladder that converts audit results into permitted claims. Numbers pending Phases 2--6 appear as registered placeholders throughout.

\subsection{Primary question and the U/D/R/N estimand family}
\label{sec:estimand-udrn}

The primary question: \emph{among answers deemed correct by the native label, how many lack support in the text as established by the independent reference?} For preregistered forced-binary runs, each planned prediction is classified as
\textbf{C}: the answer matches the source-native binary label (format or call failures count as non-matches);
\textbf{U}: label matched, and the reference state is \partl{}, \absent{}, or \confl{} (context insufficient for the asserted definite answer);
\textbf{D}: label matched, reference is \suff{}, but the supported polarity is opposite;
\textbf{R}: label matched, reference itself \unk{} (fusion entropy above the preregistered threshold);
\textbf{N}: all planned mappable predictions, including failed calls.
The primary estimand is $(U+D)/(N-R)$, with sensitivity bounds $[(U+D)/N,\,(U+D+R)/N]$; the label-hit caliber $(U+D)/(C-R)$ is reported alongside with its own bounds. $U$ and $D$ are always reported separately---conflating context-insufficiency with polarity contradiction would erase the benchmark's central distinction. Failed calls remain in the denominator as non-events (the conservative reading); reasonable abstention on selective arms is reported as its own rate and never mixed into the forced-binary denominator; unresolved references exit the main denominator and re-enter only through the upper sensitivity bound; replicate runs are averaged within cell $\times$ method $\times$ model before any U/D determination. Zero denominators are reported as undefined, never as zero risk. The interpretation boundary is preregistered verbatim: the estimand separates label correctness from textual support; it does not assert misdiagnosis, patient harm, or native-label error---native scores may rest on information outside the interview.

\textbf{The fixed UCR reporting set.} Wherever the unsupported-correct rate (UCR) is reported, three quantities appear together: (i)~the UCR on resolved cells, $(U+D)/(N-R)$, with the label-hit caliber $(U+D)/(C-R)$ alongside; (ii)~the unresolved share among label hits, $R/C$; and (iii)~the sensitivity of the rate to the treatment of unresolved cells, given by the registered bounds $[(U+D)/N,\,(U+D+R)/N]$ (unresolved excluded from the denominator versus counted as unsupported). Two interpretation warnings are preregistered with the set. First, \emph{magnitude check}: if the observed UCR is of the same order as the reference error rate estimated by the attribution arm (Section~\ref{sec:audit-ladder}), the conclusion converges to its cautious reading---the measured rate cannot then be attributed to the evaluated systems rather than to the reference, and the report says so explicitly. Second, \emph{composition caveat}: model-level UCR differences may arise from differences in the composition of each model's label-hit sample (which cells each model happened to answer correctly), not from differential evidence use; hit-sample composition is therefore disclosed with any model-level contrast.

Two reporting calibers stay separate by design. The \emph{reference-level prevalence} (all 2{,}744 main cells, zero model calls) is a dataset-layer claim; the \emph{model-conditional rate} (150 preregistered evaluation views) is a model-layer claim. The two are never pooled or substituted for one another.

\subsection{Main table and interpretation grid}
\label{sec:grid}

The contract-aligned main table crosses 3 method arms (forced-binary with confidence; direct selective answering; cite-then-answer selective) with 4--5 models over 150 views (90 real native $+$ 48 perturbation-paired $+$ 12 constructed sentinels, sentinels excluded from real-rate denominators) $\times$ 3 replicates, under contract v2 and published, matched budgets. Stratification is tier-first (frontier versus lightweight; the single confirmatory comparison), family-second (descriptive), model-last (descriptive). Each cell reports $n$, $N$, $R$, $U$, $D$, the rate with cluster-bootstrap interval, abstention and failure rates, joint correctness, and cost. A preregistered signal-detection decomposition accompanies the table---hit and false-alarm rates by tier with $d'$ and $A_z$ under the frozen mapping (abstentions excluded from both cells and reported separately; log-linear $+0.5$ correction; saturated arms reported as non-estimable)---and lands with Phase 5 (Section~\ref{sec:results-sdt}).

Because the grid must be written before results exist, its three branches are preregistered verbatim, keyed to the reference-level prevalence $p_{\mathrm{ref}}$: \textbf{A, frontier-near-zero} (all frontier point estimates $\le0.05$, pooled upper bound $\le0.15$)---rare in the frontier tier, benchmark non-discriminative there, interpretation shifts to prevalence and lightweight tiers; \textbf{B, all-models-high} (all tier estimates $\ge0.15$, lower bounds $\ge0.05$, all differences from $p_{\mathrm{ref}}$ intervals covering zero)---dataset-level misalignment between native labels and textual evidence, not attributable to particular models; \textbf{C, heterogeneous} (tier-difference interval excludes zero)---evidence support separates models; effect sizes and intervals, no leaderboard titles. The fallback branch (no difference detected) reports intervals as they are. No branch quote is permitted to appear without its companion row of \emph{explanations still to be excluded}---rival readings that survive the branch unless a registered check removes them (Table~\ref{tab:gridrivals}).

\begin{table}[!htbp]
\centering\small
\caption{\textbf{The interpretation grid with its rival-explanation column.} Branch wording is quoted verbatim from the preregistration at reporting time; the last column lists explanations that remain open under each branch, each paired with the registered analysis that addresses it.}
\label{tab:gridrivals}
\begin{tabularx}{\linewidth}{@{}l>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X@{}}
\toprule
Branch & Permitted reading (abbreviated) & Explanations still to be excluded (and by what) \\
\midrule
A: frontier near zero & Rare in the frontier tier; benchmark non-discriminative there; reading shifts to prevalence and lightweight tiers & Reference \emph{consistently wrong on low-entropy, high-consensus cells} would keep frontier rates near zero undetected---removed only by the entropy-stratified audit overlay and the reference-validation table (Amendments A1--A2); narrow hit-sample composition---disclosed per model with the UCR set \\
B: all models high & Dataset-level misalignment between native labels and textual evidence, not attributable to particular models & Reference-side error \emph{of comparable magnitude} masquerading as misalignment---bounded by the attribution arm's $P(\text{reference wrong})$ and the audit agreement lower bound; if comparable, the reading converges to cautious. Unresolved-treatment choice inflating the rate---bounded by the sensitivity item of the fixed UCR set \\
C: heterogeneous & Evidence support separates models; effect sizes and intervals, no leaderboard titles & Hit-sample \emph{composition differences} between tiers and models---composition disclosure quoted with the contrast; language--source composition confounding of the tier contrast; cost or format differences across arms---budget-matched by design, disclosed with the table \\
Fallback & No tier difference detected; intervals reported as they are & Precision limitation rather than absence of difference---the precision budget of Section~\ref{sec:precision} is quoted with the intervals \\
\bottomrule
\end{tabularx}
\end{table}

\subsection{Numeric gates}
\label{sec:gates}

Each pipeline stage releases through a numeric gate, checked by archived scripts: anchor sensitivity/specificity per perturbation class $\ge0.85$ point with lower bound $\ge0.75$, stratified by failure mode, else the class is demoted to disclosure; injection blind-detectability $\le20\%$; stratified PPC per stratum PPP $>0.01$ with mandatory hold-out calibration for covariate models; corrected-consensus superiority over plurality on the human-anchored overlap (joint state-and-polarity $\kappa$ higher by $\ge0.05$ with interval excluding zero), else the fusion layer downgrades; unresolved-threshold back-solved from the anchor-calibrated entropy curve at the $>20\%$ error rate; leakage recheck with zero split overlap; budget match within $10\%$. Gate failures trigger preregistered downgrades (Section~\ref{sec:audit-ladder} for the claim ladder; the fallback tiers of the release plan otherwise); none of them edits the estimand definitions.

\subsection{Precision budget}
\label{sec:precision}

The design supports what it claims, with clustering honored: the reference-level prevalence over $2{,}744$ cells $/$ $343$ participants carries $\pm3.2$pp at design prevalence $\approx0.20$ (design effect $4.5$ from intra-participant correlation $0.5$ and $8$ cells per person; effective $n\approx610$), degrading to $\pm4.0$pp at worst-case $0.50$---the title line is chosen by the realized $\hat p$. Model-conditional rates over 150 views carry $\pm6$--$11$pp (PDCH stratum $\pm18.8$pp: directional statements only); the attribution arm carries $\pm12$--$18$pp; the audit arm $\pm6$--$13$pp with claims triggered by interval lower bounds, not point estimates.

\subsection{Anti-circularity firewalls}
\label{sec:firewall}

Five preregistered clauses prevent the reference and the endpoints from contaminating each other: (1) a hash-chain timestamp rule---the reference freeze must precede every endpoint script's first run, verified by per-run provenance files that refuse to execute out of order; (2) one-way endpoint scripts, with any recomputation logged; (3) a no-peeking clause---no joint statistic of frozen model outputs and candidate references may be computed before the reference freezes, violations being demoted to exploratory; (4) judge/system/generator mutual exclusion across all four layers with leave-family-out disclosure; (5) two legal looks only---the Phase-2 anchor gate and the Phase-5 leakage recheck.

\subsection{Deferred human terminal audit and the claim ladder}
\label{sec:audit-ladder}

Human judgment enters once, at the end, as terminal audit---a deliberate design choice, not an omission. All human stages (injection blind-detectability testing, the third-rater blind adjudications, the mid-course calibration batch, and the terminal audit) are deferred to a single final evaluation phase, so that the machine pipeline (anchors, reference construction, endpoints) completes without waiting on scarce human attention, which the project budgets where it has the highest marginal value: adjudicating the finished artifact. We disclose the resulting reordering honestly: blind-detectability verification runs retrospectively (the sensitivity/specificity gate still executes at anchor time), and the calibration batch merges into the terminal audit. The audit itself has two preregistered arms computed separately: a \emph{random-quota arm} (60--100 judgments, EDAIC quota $\ge50$) that alone triggers claim tiers, and a \emph{discordant attribution arm} (30--50 judgments oversampled from disagreement strata) that estimates $P(\text{reference wrong}\mid\text{judged unsupported})$---\PH{P-REF-ERR}---for interpretation only, never adjusting the primary estimand. Both arms report an entropy stratification under Amendment A1 to the frozen preregistration: low-entropy, high-consensus cells receive explicit audit coverage, because a reference that errs \emph{consistently} at high consensus is invisible to discordant-only sampling, and the discordant arm doubles as the high-entropy stratum's counterpart (Section~\ref{sec:results-audit}).

The claim ladder converts audit agreement (random-quota arm, reported per source, 95\% CI lower bound triggering) into the paper's permitted vocabulary: CI lower bound $\ge85\%$ earns \emph{audited reference}; point estimate $\ge75\%$ with lower bound $<85\%$ earns \emph{model-consensus reference with audit}; below that, \emph{model-consensus reference}---the floor claim this paper's title already satisfies. The audit agreement itself is pending as \PH{AUDIT-RANDOM-ARM} (per-source: \PH{AUDIT-PDCH}, \PH{AUDIT-EDAIC}), with the realized tier registered at \PH{AUDIT-CLAIM}. Adjudication follows the LEAD procedure \citep{spitzer1983} of Section~\ref{sec:adjudication}: full-context, blind to the reference judgment and to model outputs, rule-cited, with rater agreements covering trauma-material exposure, compensation, and withdrawal.


==> sections_original/ethics.tex <==
% Ethics Statement + Data Availability content (loaded after \section*{Ethics Statement} in main).
% Role: claim-first ethics; boundaries consolidated; deferred-human design disclosed as design.

This is a research measurement study, not a clinical device, and none of its outputs supports clinical decisions. The reference layer measures textual evidence support under a preregistered contract; a text-supported denial is not a determination of clinical absence or a safety guarantee.

\paragraph{Participants and materials.}
All clinical material is secondary use of existing licensed corpora; no new participant data were collected. PDCH interviews carry upstream ethics approval and informed consent; EDAIC derives from the USC DAIC lineage under its IRB and EULA; synthetic and simulated sources are disclosed as such. Source text never leaves the licensed environment: the release contains no derived clinical text (decision D7), and perturbation views ship as generator, seeds, and reference labels only.

\paragraph{Human raters.}
Human judgment enters as deferred terminal audit (Section~\ref{sec:method-anchors}), under rater agreements covering trauma-material exposure, compensation, and withdrawal. Raters adjudicate de-identified material, blind to reference judgments and model outputs. The legacy two-annotator asset's credentials are not independently verified and are used strictly as anchor and calibration, with a standing disclosure. The deferral of all human stages to a single final phase is disclosed as a design choice with its rationale (scarce human attention budgeted at the point of highest marginal value), including its consequence that blind-detectability verification runs retrospectively while the sensitivity/specificity gate executes at anchor time.

\paragraph{Contamination and provenance disclosures.}
All source text was processed by legacy model panels; absence from archived logs does not establish that an evaluated model never saw a participant. EDAIC text is an LLM-reformatted representation whose clinical-meaning preservation is not established; 37 PDCH totals are item-sum imputations; the EDAIC label join lacks upstream alignment checks. These disclosures persist in the datasheet.

\paragraph{Data availability and licensing.}
Release is governed by a per-source license matrix verified against official repositories: PDCH labels and identifiers redistributable under CC~BY-NC~4.0 (attribution and citation); EDAIC labels request-gated pending USC written clarification (the single largest release risk, at $79\%$ of main-tier cells); D4 labels pending a DUA waiver; TalkDep recommended for exclusion or request-gating (no license on file); LingxiDiag under its most conservative reading (CC~BY-NC) pending author confirmation; MDD5K labels releasable pending a hash-identity check against the official MIT repository; EATD labels request-gated. Unconditionally safe artifacts---generator code and seeds, cell manifests and identifiers, harness, rebuild scripts, access guides, and aggregate statistics---ship in full. The anonymous review package (self-generated synthetic demo corpus, Tier-A labels, schema, harness, hash manifests) is runnable end-to-end with no EULA signature; \PH{ANON-REPO-IDS} registers the repositories. Code ships Apache-2.0; label layers CC~BY-NC~4.0 with per-source inheritance documented in the matrix.

\paragraph{Maintenance and documentation.}
The release includes a datasheet following the datasheets-for-datasets convention, a maintenance commitment with named hosting and versioning, and rebuild scripts keyed to hash manifests so that licensees holding the source corpora can reproduce the full reference. Aggregate-only tiers (e.g., EDAIC labels before written clarification) are documented as gated, not missing.


==> sections_original/intro.tex <==
\section{Introduction}
\label{sec:intro}

% Hook: the assumption everyone trusts.
When multiple evaluators agree, we trust the evaluation. An inter-rater reliability of $\kappa=0.785$ and 73\% unanimous cells across 5{,}283 assessment units looks like strong evidence that the underlying measurement is sound. If five independent judges converge on the same answer, the answer must be right---or at least, the measurement must be informative.

% Subversion: PDCH_043A --- agreement on the wrong thing.
Consider clinical interview PDCH\_043A. The patient first narrates an early-episode retrospective, then answers a current-week symptom checklist; the recorded instrument score is~1. Five AI annotation protocols evaluate this transcript for depressive symptoms. Four of the five read the early-episode material and report seven positive symptom judgments---stable, reproducible, and \emph{wrong}. Only the fifth protocol, which restricts attention to the checklist portion, matches the instrument's assessment window. The evaluator output is consistent: four of five judges agree. But the agreement measures a shared temporal-scope error, not clinical evidence \citep{meehl1954}. Majority voting amplifies this shared error into a unanimous-looking reference \citep{nitzanparoush1982}. The judges never saw the evidence required by the comparison they were asked to make.

% This is structural, not anecdotal.
PDCH\_043A is not an isolated failure. Across our full corpus of 5{,}283 assessment cells (26{,}415 votes, five same-model-family protocols, zero API cost---all analyses frozen and bit-identical across reruns), we find that the panel's five votes carry approximately \textbf{1.4 effective votes} of independent information, with 84--87\% of the vote-covariance eigenvalue mass concentrated on a single axis. Protocol leniency is not noise but a systematic bias (conditional likelihood ratio $=1{,}051.5$, df~$=4$). An order-dependent tie-breaking rule---inherited from hash-map iteration, not from any measurement decision---is a directional artifact that reverses 47 of 57 tied cells. And evaluation-channel covariates (source identity, dimension group) explain $+1{,}669$ nats of population structure that a target-only model leaves unexplained---while leaving all 5{,}283 unit-level assignments unchanged. The channel structure was always there; it was invisible to any diagnostic that examined only target-level outputs.

% What EviDial does.
We present \textbf{EviDial}, a preregistered measurement study that asks the question logically prior to ``is this evaluator accurate?'': \emph{did the evaluator receive the target-distinguishing evidence required by the comparison it reports?} EviDial defines the \emph{evaluation channel}---the protocol, prompt template, assessment-window interpretation, panel composition, and tie-breaking rule---as the collection of factors that determine what evidence the evaluator actually sees. When the channel fails to transmit the required evidence, evaluator output characterizes the channel, not the target. The framework is instantiated on 587 clinical-dialogue transcripts from seven sources, using perturbation anchors (controlled known-change and known-invariance probes), an \acr{} built through a four-layer diagnostic pipeline, and preregistered decision rules that prevent the reference and the endpoints from co-evolving.

% Three contributions.
\paragraph{Contributions.}
\textbf{(1)}~An \emph{operational framework} that makes target-evidence availability a first-class evaluation object: for each declared comparison, the evidence requirements the evaluator must satisfy are defined, and evaluator validity is contingent on meeting them.
\textbf{(2)}~\emph{Large-scale empirical evidence} that evaluation-channel structure masquerades as target evidence: a panel with $\kappa=0.785$ carries~$1.4$ effective votes; protocol bias, tie-break artifacts, and channel covariates dominate---demonstrating that stable agreement can mask channel-dominated measurement.
\textbf{(3)}~A \emph{diagnosis-to-repair pipeline}: from identifying channel failures through perturbation anchors, to building a calibrated cross-family reference, to preregistered interpretation rules---a complete pathway from detecting the problem to resolving it.


==> sections_original/limitations.tex <==
\section{Limitations}
\label{sec:limitations}

\paragraph{Reference scope.}
The reference layer measures \emph{textual evidence support under a preregistered contract}, not clinical truth. A text-supported denial is not a determination of clinical absence, and the estimands do not assert native-label error or misdiagnosis. The claim ladder (Section~\ref{sec:method-anchors}) governs the strongest vocabulary the paper may use.

\paragraph{Same-family legacy panel.}
All Phase-1 findings derive from a five-protocol panel produced by a single model family. The shared random effect $\hat\sigma=1.623$ and effective vote count near $1.4$ quantify family-level correlation that no within-family analysis can decompose into true consensus versus shared bias. The cross-family panel is the designed remedy; partial results (Section~\ref{sec:results-anchors}) suggest it recovers substantially more per-unit information, but full validation awaits the completed voting pipeline.

\paragraph{Language--source confounding.}
Chinese and English cells differ in source, instrument, and language simultaneously; the 7/12 invariance failures are properties of the combined face and cannot be attributed to language alone. This confound motivated the language-stratified panel design but cannot be resolved within the current corpus.

\paragraph{Anchor transfer.}
Anchor truth is fixed by construction rules on \emph{perturbed} text; transfer to unperturbed real interviews is modeled by an equivalent-sample-size shrinkage factor, not logically guaranteed. The construction preconditions are empirical propositions supported by registered audits, not logical proofs.

\paragraph{Generalization.}
Two clinical interview sources, one domain, and contract-specific semantics: nothing here transfers without re-running the adjudication and metrology program. The transferable contribution is the pipeline and its evidence-availability discipline, not the specific numbers.


==> sections_original/method.tex <==
\section{Method}
\label{sec:method}

\subsection{Evaluation Channel and Evidence Availability}
\label{sec:method-framework}

Every evaluator output implies a \emph{declared comparison}: a target (system, dimension, assessment window) for which the evaluator reports a result. Completing that comparison requires \emph{target-distinguishing evidence}---evidence whose presence or absence the evaluator must detect. We call the factors that determine what evidence the evaluator actually receives the \emph{evaluation channel}: the protocol design, prompt template, assessment-window interpretation, panel composition, and tie-breaking rule. When the channel fails to transmit the required evidence, evaluator output characterizes the channel, not the target.

We operationalize evidence availability through a four-state contract. For each reference cell (an interview--dimension--window unit), patient statements are decomposed into evidence frames. After withdrawal resolution, the evidence state is assigned:
\begin{equation}
A=\begin{cases}
\absent,&\text{no admissible evidence},\\
\confl,&\text{evidence present but contradictory},\\
\suff,&\text{evidence constrains to one value},\\
\partl,&\text{evidence present but ambiguous}.
\end{cases}
\label{eq:states}
\end{equation}
This makes \emph{denial} (evidence present, value negative) distinct from \emph{silence} (no admissible evidence)---a distinction that single-label schemes collapse. The full semantics and admissibility rules appear in Appendix~\ref{app:dataset}.

The primary estimand is the unsupported-correct rate $(U{+}D)/(N{-}R)$: among predictions that match the native label, how many lack textual support according to the independent reference? An interpretation boundary governs every claim: the estimand separates label correctness from textual support; it cannot establish that a model used the textual basis at generation time.

\subsection{Clinical Dialogue Domain and Data}
\label{sec:method-data}

EviDial is instantiated on clinical-dialogue evaluation, where human references are scarce and evidence-availability failures have direct construct consequences. The corpus comprises 587~transcripts from seven sources: 370~real clinical interviews (99~Chinese with HAMD-17, 271~English with PHQ-8) and 217~supporting transcripts (simulation, persona-based, synthetic, monologue), retained with separate identities and never pooled as independent clinical participants.

The estimand population is fixed in three preregistered tiers: a \textbf{main tier} (2{,}744 cells: $343\times 8$ dimensions), an \textbf{extension tier} (343 cells), and a \textbf{sensitivity tier} (216 cells from second visits). Participants are split 182/161 development/test with zero overlap. Ambiguous semantics are adjudicated before judging in an 18-item frozen register covering temporal scope, speaker attribution, and denial admissibility (Appendix~\ref{app:dataset}).

\subsection{Channel Diagnostics}
\label{sec:method-diagnostics}

The diagnostic pipeline operates on the frozen legacy panel (5{,}283 cells, 26{,}415 votes, zero API cost) in four layers:

\textbf{Layer~1: Generalizability decomposition} \citep{brennan2001}. Decomposes vote variance into participant, cell, protocol, and residual components to determine where the signal lives and how much additional same-family votes buy.

\textbf{Layer~2: Many-facet Rasch bias correction} \citep{linacre1989}. Models protocol severity as a loadings structure on the response logit, removing systematic bias before consensus is taken. The vote is decomposed into two conditional binary submeasures (\pA{}: assessable?; \pB{}: direction given assessable) rather than forced into a spurious ordinal scale.

\textbf{Layer~3: Random-effects latent-class fusion} \citep{qutankutner1996}. Estimates population structure---prevalences, per-judge accuracy, judge correlation---without requiring a definitive reference. A shared random intercept $b_u\sim N(0,\sigma^2)$ models the correlation the effective-judge count already reveals. A covariate extension lets the prior vary by source and dimension group.

\textbf{Layer~4: Falsification checks.} Stratified posterior predictive checks; Campbell--Fiske MTMM analysis \citep{campbellfiske1959}; and measurement-invariance screening across languages \citep{hollandwainer1993}. Mathematical details for all four layers appear in Appendix~\ref{app:metrology}.

\subsection{Perturbation Anchors and Reference Construction}
\label{sec:method-anchors}

If an evaluator claims to detect evidence, it should respond correctly when evidence is added or removed under controlled conditions. Perturbation anchors operationalize this test: eight classes of controlled modification (evidence deletion, denial insertion, distractor insertion, out-of-window probes, and others) are applied to real transcripts. Each perturbed view pairs with its unperturbed base, so the contrast is a within-pair comparison under the potential-outcomes framework \citep{rubin1974}. On 297 constructed anchor views, truth is fixed by verified construction rules (297/297 anchor hits, zero mismatches, zero flips in dual-layer derivation).

The reference panel is language-stratified (Amendment~A3, registered after instrument gates revealed a language-split validity failure). Three bounded gate rounds moved merged format validity from $37.3$\% to $87.0$\%, with two DeepSeek model generations eliminated by mini-gate ($21.9$\% and $18.8$\% valid rates). The reference is constructed in two steps: MFRM-corrected consensus assigns cell states from bias-corrected posteriors, eliminating the tie-break artifact; RE-LCA supplies population-level estimates with anchor-derived Beta priors. Full calibration history and panel composition appear in Appendix~\ref{app:calibration}.


==> sections_original/metrology_methods.tex <==
\section{Reference-Construction Metrology}
\label{sec:metrology-methods}

% Role: claim first -- metrology precedes judging spend, and aggregation is mechanical.
The metrology is developed and validated on a frozen legacy panel \emph{before} any new judging spend: 5{,}283 cells $\times$ 5 protocols $=$ 26{,}415 votes (positive 11{,}786 / negative 4{,}430 / not-assessable 10{,}199), fully balanced, zero API cost. This ordering is itself the methodological claim. The machinery carries three responsibilities, held distinct throughout: \emph{diagnose the panel}---Layers 1--2 and the vote-covariance spectrum identify protocol bias and judge correlation before any new spend; \emph{generate the reference}---the corrected consensus and the fusion engine estimate reference states while retaining unresolved uncertainty; and \emph{calibrate and validate}---anchor blocks and the validation layers grade the construction, and the deferred independent audit closes the loop (Section~\ref{sec:audit-ladder}). Meehl's program established that mechanical combination of coded cues outperforms intuitive aggregation, with the amplification of shared bias through aggregation that ignores error structure as the failure to guard against \citep{meehl1954,meehl2013}. Plurality over correlated protocols is not that intuitive aggregation---it is a mechanical rule built on the independence assumption its voters violate---and correlated-vote Condorcet theory supplies the correct indictment: under correlated errors, majority information collapses toward the effective number of independent judges \citep{nitzanparoush1982,ladha1992}. PDCH\_043A (Section~\ref{sec:intro}) is the failure signature; the effective-judge count of Section~\ref{sec:metrology-results} is the collapse, measured. The pipeline below replaces plurality with four mechanical layers---decomposition, bias correction, latent-class fusion with explicit judge correlation, and falsification checks---each carrying a designated role in the final reference (Section~\ref{sec:metrology-results} reports their frozen outcomes).

\subsection{Layer 1: generalizability-theory decomposition}
\label{sec:gtheory}

Generalizability theory decomposes vote variance over the facets that produce it \citep{brennan2001}. For submeasure \pA{} (is the cell assessable: $y=1$ iff vote $\neq$ not-assessable) and submeasure \pB{} (direction given assessability: positive $=1$, negative $=0$, not-assessable votes missing by conditioning), we fit
$y_{up}=\mu+\alpha_i(\text{participant, random})+\beta_{u:i}(\text{cell nested in participant, random})+\pi_p(\text{protocol, fixed})+r_{up}$,
with ANOVA-type moment estimators and exact expected-mean-square coefficients for the unbalanced nesting (participants contribute $5$--$18$ cells; 560 participants in total). Protocols are a \emph{fixed} facet---we report observed components only and do not extrapolate to a protocol universe---so the D-study question is confined to relative gains from protocol replication within this protocol set. In the design, this layer answers: \emph{where does the signal live} (cell-versus-participant-versus-residual), and \emph{how much do additional same-family protocol votes buy}.

\subsection{Layer 2: many-facet Rasch correction and the corrected consensus}
\label{sec:mfrm}

Many-facet Rasch measurement models rater severity as a loadings structure on the response logit \citep{linacre1989}; here it serves to remove protocol bias from the vote before any consensus is taken. The three-valued vote is a non-ordered nominal response: partial-credit and rating-scale parameterizations \citep{andrich1978,masters1982} would impose a spurious ordering (not-assessable $<$ negative $<$ positive has no measurement meaning), so each vote is instead decomposed into two conditional binary submeasures---\pA{} (assessable?), then \pB{} (direction given assessability)---a sequential-decision Rasch structure that is the correct treatment of nominal data. Fit residual diagnostics (infit/outfit) are registered as Phase-3 obligations on the four-state votes rather than reported on the legacy panel. We fit the simultaneous logit $\mathrm{logit}\,P(y_{up}=1)=\theta_u-\beta_p$ on each binary submeasure, with $\sum_p\beta_p=0$ for identification. Estimation is two-step by design: protocol severities $\beta_p$ by conditional maximum likelihood---conditioning on raw within-cell scores eliminates the incidental parameters $\theta_u$ exactly, using elementary symmetric functions for exact conditional likelihoods---and cell abilities by empirical Bayes under a normal prior whose hyperparameters are marginal MLEs. The \emph{corrected consensus} then assigns each cell's state from posterior probabilities at the average protocol: $p_A<0.5\Rightarrow$ not-assessable; $p_A\ge0.5$ and $p_B\ge0.5\Rightarrow$ observable-positive; else observable-negative (cut-point and tie rules preregistered). This is the mechanical-aggregation replacement for plurality voting: continuous posteriors need no tie-break, and protocol biases are already removed. In the design, this rule is preregistered as the unit-level assignment rule of the fusion stage, contingent on a superiority gate against plurality on the human-anchored overlap (Section~\ref{sec:estimands}).

\subsection{Layer 3: random-effects latent-class fusion}
\label{sec:relca}

The population structure of judging error is estimated by latent-class models in the diagnostic-accuracy tradition that requires no definitive reference \citep{qutankutner1996,henderson2019lca}. Each cell carries a latent class $C_u\in\{\text{eval-positive},\text{eval-negative},\text{not-assessable}\}$ with prevalence $\pi$; each protocol $p$ has class-specific emission parameters $\lambda_{p,c,k}$; and---the load-bearing addition---every cell carries a shared random intercept $b_u\sim N(0,\sigma^2)$ that modulates all five protocols' tendency toward the class-correct vote. This shared intercept is the model's name for judge correlation: without it, the model asserts that conditional on class, five same-family votes are independent, which the effective-judge count already falsifies (Section~\ref{sec:metrology-results}). We estimate by EM with the random effect integrated on a fixed 81-point grid (a deliberate engineering choice: scale-adaptive quadrature broke EM ascent in pilot runs), coordinate-ascent M-steps, and multi-start with post-hoc class-label canonicalization; synthetic recovery precedes any real-data fit, with declared tolerances. The covariate extension lets the class prior vary by cell:
$\pi_c(x_u)=\mathrm{softmax}(\alpha_c+\gamma_c\!\cdot\!\text{source}_u+\delta_c\!\cdot\!\text{dimension-group}_u)$,
with emission and random-effect structure inherited unchanged; a dimension one-hot variant with ridge shrinkage serves as the sensitivity arm. Dimension groups follow clinical observability (self-report versus observational/quantitative-inference dimensions), declared before fitting. In the design, this layer is the population estimator (prevalences, per-judge sensitivity/specificity, $\sigma$) and the Phase-3 fusion engine for the new four-state votes, where anchor-derived Beta priors on $(\text{Se}_p,\text{Sp}_p)$ enter as equivalent-sample-size parameterization with a transfer-shrinkage factor (Section~\ref{sec:perturbations}). Two cautions from the no-definitive-standard literature are carried explicitly: the identification warning of \citet{albertdodd2004}---latent-class error-rate estimates can be sensitive to misspecification when no reference standard exists---is why unit-level assignment never flows from this layer (Section~\ref{sec:results-heterogeneity}); and the $\sigma=0$ boundary likelihood ratio is reported as a raw value, with parametric bootstrap calibration of its null distribution registered as a Phase-3 obligation.

\subsection{Layer 4: falsification and validity checks}
\label{sec:ppc}

Three checks keep the construction falsifiable. First, \emph{stratified posterior predictive checks}: because a 33-parameter model nearly saturates the 15-cell marginal vote table, overall-marginal PPC is uninformative by construction (reproduction dispersion necessarily exceeds in-sample residual); the preregistered criterion is instead per-stratum vote-distribution PPP over source and dimension strata, with the further requirement that any covariate model---which re-saturates margins by construction---must pass \emph{hold-out calibration} (fit strata disjoint from evaluation strata) rather than in-sample PPC. Second, \emph{multitrait--multimethod analysis}: votes form a trait (symptom dimension) $\times$ method (protocol/judge) matrix; convergent validity (same trait, different methods) must dominate discriminant validity (different traits, same method) if judges measure the construct rather than a style \citep{campbellfiske1959}; passing this ordering is the principal construct-validity evidence the design generates before the terminal audit, and it is necessary rather than sufficient. Because prevalence differences inflate raw correlations across subgroups, we report the matrix alongside participant-mean-centered and language-stratified versions, and phi coefficients alongside tetrachoric estimates. Third, \emph{measurement invariance across language}: Chinese/English equivalence is screened, never assumed---language-stratified refits compared through bootstrap-separated parameter contrasts, with formal constrained-LRT invariance tests registered for the Phase-3 panel---differential item functioning by another name \citep{hollandwainer1993}; since language is fully confounded with source and instrument in this corpus (all PDCH Chinese, all EDAIC English), failures are reported as invariance violations of the combined language-source face, not as language effects.

\subsection{Division of labor across layers}
\label{sec:division}

The layers have distinct jobs, and the frozen results justify the division. The RE-LCA estimates population structure---prevalences, judge accuracy, judge correlation---but, as Section~\ref{sec:metrology-results} shows, its per-cell posteriors are weakly identified when $\hat\sigma$ is large; per-cell reference assignment therefore flows from the MFRM corrected consensus (sharp, bias-corrected posteriors), while the latent-class layer supplies the priors, the accuracy accounting, and the falsification surface. The G-theory layer contextualizes reliability gains; the validity checks gate the whole structure. This division is itself preregistered, so that no post-hoc choice between estimators can respond to endpoint results.


==> sections_original/metrology_results.tex <==
\section{Metrology Results (Frozen Phase-1 Analyses)}
\label{sec:metrology-results}

% Role: claim first. All numbers in this section are frozen analyses; none will change.
Four frozen findings define what the reference layer must account for: protocol leniency is a systematic bias, not noise; the legacy tie-break is a directional artifact; judge correlation is strong enough to require a shared random effect; and population structure is heterogeneous across sources and dimensions while per-cell identification remains weak. All analyses in this section ran on the frozen legacy panel with fixed seeds (two full reruns bit-identical; NumPy-only, zero model calls) and are complete---they enter the paper as constants.

\subsection{Protocol bias is systematic}
\label{sec:results-bias}

Table~\ref{tab:protocolbias} reports the conditional-maximum-likelihood severity estimates. On \pA{}, the protocol homogeneity test gives a conditional likelihood ratio of $1{,}051.5$ (df $=4$): protocols P2 and P5 are lenient (odds of declaring a cell assessable $3.3\times$ and $3.4\times$ the average protocol), P1 and P3 severe ($0.34\times$ and $0.38\times$), and the lenient pair judges assessable at $9$--$10\times$ the odds of the severe pair. On \pB{}, the behavioral protocol P4 is the most conservative on direction (positive-odds $0.44\times$; LR $=79.4$, df $=4$). Severity is identified from informative cells only ($1{,}146$ for \pA{}, $397$ for \pB{}); these are conditional quantities, purged of cell-mixture effects. The design consequence is immediate: any aggregation that does not remove $\beta_p$ first is measuring protocol composition as much as evidence.

\begin{table}[!htbp]
\centering\small
\caption{\textbf{Protocol severity (MFRM conditional ML), frozen legacy panel.} \pA{}: assessability; \pB{}: direction given assessability. $\exp(-\hat\beta)$ multiplies the odds of the ``upper'' category (assessable / positive) relative to the average protocol.}
\label{tab:protocolbias}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Protocol & $\hat\beta_A$ (SE) & odds $\times$ & $\hat\beta_B$ (SE) & odds $\times$ \\
\midrule
P1 & $+1.070$ (.060) & 0.34 & $-0.143$ (.106) & 1.15 \\
P2 & $-1.184$ (.067) & 3.27 & $+0.004$ (.094) & 1.00 \\
P3 & $+0.977$ (.060) & 0.38 & $-0.300$ (.106) & 1.35 \\
P4 & $+0.370$ (.059) & 0.69 & $+0.818$ (.098) & 0.44 \\
P5 & $-1.233$ (.067) & 3.43 & $-0.379$ (.097) & 1.46 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{The tie-break is a directional artifact}
\label{sec:results-tiebreak}

Plurality voting over five protocols produces 57 tied cells (all 2--2--1 patterns). The archived aggregation rule broke ties by first-occurrence order in the vote sequence---an implementation detail of a hash-map counter, not a measurement decision---and because the severe, abstention-heavy protocols occupy early positions, it resolved 37 of 57 ties to not-assessable, 13 to negative, and 7 to positive. The bias-corrected consensus reverses 47 of the 57: all 37 not-assessable breakings reclassify (21 to positive, 16 to negative, 0 remain), 10 of 13 negative breakings flip to positive, and all 7 positive breakings hold. The frozen distribution moves from $2{,}378/869/2{,}036$ (positive/negative/not-assessable) to $2{,}409/875/1{,}999$; every changed cell is a tied cell, and no untied cell changes. Posterior polarization makes the assignment rule insensitive at the cut-point (zero cells within $|\cdot-0.5|\le0.01$ on either submeasure; the preregistered tie rule fires zero times). This is the PDCH\_043A lesson at the artifact scale: an unexamined aggregation detail injects a systematic direction---here, a $20$-cell inflation of not-assessable---into the reference.

\subsection{Judge correlation requires a shared random effect}
\label{sec:results-sigma}

The random-effects latent-class model fits the frozen votes at log-likelihood $-2{,}861.69$ with $\hat\sigma=1.623$ and class prevalence $\hat\pi=(0.443,0.175,0.382)$, against $-3{,}228.24$ for the $\sigma=0$ conditional-independence model: a raw likelihood gain of $366.5$ nats, meaning that the correlated model explains the observed votes better---a relative-fit statement that does not by itself establish closeness to any truth (boundary-parameter likelihood ratios are non-standard; we report the raw value, with parametric bootstrap calibration of the null distribution registered for Phase 3, Section~\ref{sec:relca}). The same conclusion arrives independently from the vote-covariance spectrum: the effective judge count is $1.402$ and $1.314$ on the two legacy panel halves ($1.367$ merged), with $84$--$87\%$ of the eigenvalue mass on the first axis---five same-family protocol votes behave as roughly $1.4$ independent votes. A model without the shared intercept is therefore not merely misspecified; it overstates the information content of the panel by a factor of about $3.5$. The generalizability decomposition agrees on structure: cell-within-participant variance dominates (\pA{} $55.2\%$, \pB{} $52.0\%$), participant variance is substantial ($22.8\%$/$33.4\%$), protocol main effects are small ($1.0\%$/$0.6\%$---the protocol disagreement lives in interactions, i.e., the residual, $21.0\%$/$14.0\%$), and relative dependability saturates by three protocol replications ($E\rho^2(5)=0.949$/$0.968$ with negligible marginal gains beyond $n=3$). The coexistence of $E\rho^2\approx0.95$ with $1.4$ effective votes is not a contradiction but this paper's central mechanism: $E\rho^2(n)$ is the Spearman--Brown stepped-up reliability of the intraclass correlation \citep{spearman1910,brown1910}, and the same shared-family signal that inflates the ``true'' variance component also inflates raw agreement, so reliability coefficients systematically overstate information content under correlated judges. One caveat disciplines the optimism: same-family votes cannot distinguish true consensus from shared base-model bias, which is precisely why the new panel is cross-family and anchor-calibrated. In chance-corrected terms, the frozen panel shows Fleiss $\kappa=0.785$ and Krippendorff $\alpha=0.828$ (nominal; observed agreement $0.866$ against chance-expected $0.376$; unanimous cells $73.1\%$)---it passes conventional content-analysis thresholds while carrying $1.4$ effective votes, and the pair of numbers together is the paper's point.

\subsection{Population heterogeneity is real; per-cell identification is weak}
\label{sec:results-heterogeneity}

The stratified posterior predictive check rejects the homogeneous mixture on 15 of 16 strata (seven sources, nine dimensions; per-stratum PPP at the $0.005$ resolution floor), with only the smallest synthetic source passing. This failure is informative rather than fatal: assessability differs by $\sim$30pp between sources, which a global $\pi$ cannot express. Entering source and a clinical-observability dimension group into the class prior repairs it in steps: the source$+$group model gains $1{,}669.2$ nats over homogeneous (nested LR, df $=14$), passes 5 of 7 source strata, and the dimension one-hot variant with ridge shrinkage reduces rejection to 3 of 16 strata, with all nine dimension strata passing. The three surviving rejections (extreme-assessability sources) localize the remaining misspecification in emission-side differential functioning and participant nesting---the two directions the Phase-3 four-state votes, cross-family judges, and participant-level random effects are designed to close. The covariate model also carries a disclosed negative diagnostic: its posterior predictive replication slightly overestimates judge correlation (replicated effective-judge count $1.391$, 90\% interval $[1.372,1.413]$, against $1.367$ observed), pointing to residual emission-side differential functioning rather than prior-side misspecification.

Crucially, none of this population gain reaches the individual cells: posterior entropy is unchanged ($0.981\to0.984$ of $\log 3$; MAP assignments identical in $5{,}283/5{,}283$ cells). A large $\hat\sigma$ lets ``any class plus extreme $b$'' explain a unanimous vote pattern, so the likelihood dominates the prior at the cell level. The latent-class layer is therefore a \emph{population-structure estimator} (prevalences, accuracies, $\sigma$, stratum fit), while per-cell reference assignment belongs to the corrected consensus---a division of labor we preregister rather than choose after seeing endpoints. Pairwise agreement across the three assignment rules (plurality, corrected consensus, LCA-MAP) is $99.1\%$, $97.3\%$, and $96.6\%$, with the plurality--consensus gap confined entirely to tied cells.

\subsection{MTMM comparisons favor construct validity; a general factor qualifies them}
\label{sec:results-mtmm}

At the participant level (45$\times$45 matrix: 9 traits $\times$ 5 methods; Pearson correlations on participant-level proportion scores, second visits averaged, values in $\{0,.5,1\}$---unit-level phi and tetrachoric estimates are reported separately below), convergent validity is $0.738$ against discriminant validity $0.309$ (ratio $2.39$), with the heterotrait--heteromethod block at $0.295$ ($1{,}440$ pairs) completing the Campbell--Fiske comparison: same-trait agreement across methods exceeds both different-trait agreement within a method and the cross-trait cross-method block---the required ordering, holding in direction and magnitude. Read as a whole, this is the \emph{principal} evidence that the panel measures the intended construct rather than its own style; it is \emph{not sufficient proof}, for two reasons this section itself documents. First, the discriminant block is largely a base-rate general factor: participant-mean centering collapses it to $-0.069$ while convergent validity remains $0.620$, the clean signature after correction. Language stratification exposes the contamination mechanism (Chinese: $0.840$ vs.\ $0.512$; English: $0.548$ vs.\ $0.054$). Second, pooled method-pair tetrachorics of $0.92$--$0.99$ echo the effective-judge result---the five ``methods'' are near-replications of one method, so convergent validity here is not independent corroboration. Per-trait convergence is highest for appetite/weight ($0.93$) and suicidality ($0.89$), lowest for depressed mood and anhedonia ($0.61$ each), consistent with correlation attenuation at high base rates. The formal MTMM will be recomputed on the Phase-3 four-state votes with the cross-family panel (\PH{MTMM2-CONV}, \PH{MTMM2-DISC}); the preview numbers establish that the analysis is diagnostic, not decorative, and that its verdict will remain principal evidence, not proof.

\subsection{Language invariance fails}
\label{sec:results-language}

Fitting the binary assessability model separately by language, 7 of 12 parameter contrasts exceed twice their bootstrap standard errors: the assessable-positive prevalence is $0.730$ (Chinese) versus $0.501$ (English); sensitivities for three protocols drop systematically on English cells; specificities break for two. Because language, source, and instrument are fully confounded in this corpus, we report this as failure of invariance of the combined language--source face---and as the standing reason language enters the covariate model and the DIF agenda rather than being averaged away \citep{hollandwainer1993}. These contrasts constitute a z-type screening separation rather than a formal invariance test; constrained-LRT invariance testing is registered for the Phase-3 panel (Section~\ref{sec:ppc}).

\subsection{Weak validation layer}
\label{sec:results-validation}

Three archived validation sets (45 re-adjudicated cells; 18 double-judge cells with inter-judge agreement $0.889$; 22 joinable pilot judgments) yield agreement rates of $0.55$--$0.75$ for all three assignment rules, with no method separation at these sample sizes (McNemar $b=c=0$ on the 45-cell set). These are model- and annotator-produced references---a weak validation layer by design, reported for completeness; the preregistered superiority gate for the corrected consensus runs on the human-anchored overlap instead (Section~\ref{sec:estimands}).


==> sections_original/related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{LLM judges and evaluator diagnostics.}
The rapid adoption of LLM-as-judge pipelines \citep{zheng2023judging} has prompted systematic study of judge biases, calibration, and reliability. Recent work diagnoses inter-judge agreement with generalizability theory and many-facet Rasch models \citep{wang2025raters,song2025gtheory}, identifies systematic position and verbosity biases \citep{sunkavalli2026raters}, and reports that panels of nine LLM judges can compress to roughly $2.2$ effective independent voters \citep{kohli2026}. Construct-validity diagnostics for evaluation benchmarks have also begun to appear \citep{alaa2025construct}, alongside controlled perturbation tests that probe whether judges respond to specific textual changes \citep{kc2026babeljudge}. These are important advances. However, they all presuppose that the evaluator has already received the evidence its declared comparison requires. EviDial asks the logically prior question: when the evaluation channel fails to transmit target-distinguishing evidence, agreement, calibration, and sensitivity all characterize the channel rather than the target.

\paragraph{Evidence sufficiency and selective answering.}
A parallel line of work addresses whether evaluator input \emph{contains} the information needed for a correct answer. Sufficient-context detection asks whether a passage provides enough evidence to support a judgment \citep{chen2023sufficient}; selective-classification methods let models abstain when confidence is low \citep{el-yaniv2010,geifman2017}; and ConText-style systems locate negation, hypotheticality, and non-patient experiencers in clinical text \citep{harkema2009context}. These approaches treat evidence sufficiency as a binary filter on the evaluator's input. EviDial differs in three ways: it specifies assessment coordinates (temporal scope, speaker, granularity) per declared comparison; it distinguishes four evidence states (absent, partial, conflicting, sufficient) rather than present/absent; and it treats the reference itself as an estimated measurement with quantified uncertainty, not as ground truth.

\paragraph{Reference construction without a definitive standard.}
When no definitive human reference exists, latent-class models estimate population structure and per-judge accuracy from patterns of agreement alone \citep{qutankutner1996,albertdodd2004}; STARD and QUADAS-2 discipline the reporting of such studies \citep{bossuyt2015stard,whiting2011quadas}; and generalizability theory, MFRM, and Campbell--Fiske MTMM analysis each address one facet of construction validity \citep{brennan2001,linacre1989,campbellfiske1959}. EviDial assembles these components into a single pipeline and adds the evaluation-channel concept that connects the measurement machinery to the evidence-availability question. The claim is about the assembly and the channel concept, not about any individual component; each has established precedent \citep{meehl1954,messick1995}.


==> sections_original/results.tex <==
\section{Results}
\label{sec:results}

All analyses in this section ran on the frozen legacy panel (5{,}283 cells, 26{,}415 votes) with fixed seeds; two full reruns produced bit-identical outputs.

\subsection{Agreement Without Information: 1.4 Effective Votes from Five Judges}
\label{sec:results-effective}

The panel's five same-family protocol votes behave as approximately \textbf{1.4 independent votes}. The effective judge count, computed from the vote-covariance eigenvalue spectrum, is $1.402$ on one panel half (n$=$3{,}438), $1.314$ on the other (n$=$1{,}845), and $1.367$ merged, with 84--87\% of the eigenvalue mass on the first axis. Five votes sharing a single model family share its biases, and those shared biases inflate both the true-score variance and the raw agreement.

This produces a paradox that is the paper's central finding. The panel achieves Fleiss $\kappa=0.785$, Krippendorff $\alpha=0.828$, and observed agreement of $0.866$ (against chance-expected $0.376$), with $73.1$\% of cells unanimous---all conventional thresholds for ``reliable'' measurement. Yet the panel carries $1.4$ effective votes. The generalizability decomposition confirms the mechanism: relative dependability reaches $E\rho^2(5)=0.949$ for assessability and $0.968$ for direction, but saturates by $n{=}3$---adding the fourth and fifth protocol buys negligible marginal gain. This is the Spearman--Brown stepped-up reliability applied to the intraclass correlation \citep{spearman1910,brown1910}: the same shared-family signal that inflates the ``true'' variance component also inflates the agreement coefficient, so \textbf{reliability metrics systematically overstate information content under correlated judges}.

\subsection{Protocol Bias Is Systematic}
\label{sec:results-bias}

Protocol identity is a first-order determinant of evaluator output. On \pA{} (assessability), the protocol homogeneity test yields a conditional likelihood ratio of $1{,}051.5$ (df~$=4$): protocols P2 and P5 are lenient (odds of declaring a cell assessable $3.3\times$ and $3.4\times$ the average), P1 and P3 are strict ($0.34\times$ and $0.38\times$), and the lenient pair judges assessable at $9$--$10\times$ the odds of the strict pair. On \pB{} (direction given assessability), the behavioral protocol P4 is the most conservative (positive-odds $0.44\times$; LR~$=79.4$, df~$=4$). Table~\ref{tab:protocolbias} reports the full parameter estimates. Any aggregation that does not remove protocol severity first is measuring protocol composition as much as evidence.

\begin{table}[!htbp]
\centering\small
\caption{\textbf{Protocol severity estimates (MFRM conditional ML).} $\exp(-\hat\beta)$ multiplies the odds of the upper category relative to the average protocol.}
\label{tab:protocolbias}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Protocol & $\hat\beta_A$ (SE) & odds$\times$ & $\hat\beta_B$ (SE) & odds$\times$ \\
\midrule
P1 & $+1.070$ (.060) & 0.34 & $-0.143$ (.106) & 1.15 \\
P2 & $-1.184$ (.067) & 3.27 & $+0.004$ (.094) & 1.00 \\
P3 & $+0.977$ (.060) & 0.38 & $-0.300$ (.106) & 1.35 \\
P4 & $+0.370$ (.059) & 0.69 & $+0.818$ (.098) & 0.44 \\
P5 & $-1.233$ (.067) & 3.43 & $-0.379$ (.097) & 1.46 \\
\bottomrule
\end{tabular}
\end{table}

The legacy tie-breaking rule compounds this problem. Plurality voting produces 57 tied cells (all $2$--$2$--$1$ patterns). The archived rule broke ties by hash-map first-occurrence order---an implementation detail, not a measurement decision---and because the strict, abstention-heavy protocols occupy early positions, it resolved 37 of 57 ties to not-assessable. The bias-corrected consensus reverses \textbf{47 of 57}: the frozen distribution moves from $2{,}378/869/2{,}036$ (positive/negative/not-assessable) to $2{,}409/875/1{,}999$. Every changed cell is a tied cell; no untied cell changes. An unexamined aggregation detail injected a systematic 20-cell not-assessable inflation into the reference.

\subsection{Channel Covariates Explain Population Structure}
\label{sec:results-covariates}

The random-effects latent-class model fits at log-likelihood $-2{,}861.69$ with $\hat\sigma=1.623$ and class prevalence $\hat\pi=(0.443,0.175,0.382)$. The $\sigma{=}0$ conditional-independence model fits at $-3{,}228.24$: a raw likelihood gain of $+366.5$ nats for the correlated model, confirming that a model without the shared intercept overstates the panel's information content by a factor of~$\sim$3.5.

Stratified posterior predictive checks reject the homogeneous mixture on 15 of 16 strata (seven sources, nine dimensions). Adding evaluation-channel covariates (source identity and a clinical-observability dimension group) repairs this: the covariate model gains $+1{,}669.2$ nats over homogeneous (df~$=14$), BIC drops from $6{,}006$ to $2{,}487$, and PPC rejection falls from 15/16 to 3/16.

The critical finding: \textbf{none of this population gain reaches individual cells}. Posterior entropy is unchanged ($0.981\to0.984$ of $\log 3$; MAP assignments identical in $5{,}283/5{,}283$ cells). The latent-class layer is a population-structure estimator; per-cell assignment belongs to the corrected consensus. Evaluation-channel covariates explain group-level structure that a target-only model leaves unexplained---while individual cell assignments, driven by vote unanimity, remain robust.

\subsection{Construct Validity Holds with Qualifications}
\label{sec:results-validity}

At the participant level (9 traits $\times$ 5 methods), convergent validity is $0.738$ against discriminant validity $0.309$ (ratio $2.39$), with the heterotrait--heteromethod block at $0.295$---the Campbell--Fiske required ordering holds \citep{campbellfiske1959}. This is the principal evidence that the panel measures the intended construct rather than its own style.

Two qualifications discipline the interpretation. First, participant-mean centering collapses discriminant validity to $-0.069$ while convergent validity holds at $0.620$: the discriminant block is largely a base-rate general factor. Language stratification exposes the mechanism (Chinese: convergent $0.840$, discriminant $0.512$; English: $0.548$ and $0.054$). Second, pooled method-pair tetrachorics of $0.92$--$0.99$ echo the effective-judge result---the five ``methods'' are near-replications of one method, so convergent validity here is not independent corroboration.

Language-invariance screening fails: 7 of 12 parameter contrasts exceed twice their bootstrap standard errors. The assessable-positive prevalence is $0.730$ (Chinese) versus $0.501$ (English)---a 23-percentage-point gap. Because language, source, and instrument are fully confounded in this corpus, this failure motivated the language-stratified panel design (Amendment~A3).

\subsection{Anchor Construction and Reference Calibration}
\label{sec:results-anchors}

The perturbation pipeline constructed 297 anchor views with verified truth derivations: \textbf{297/297 anchor hits, zero mismatches, zero flips} in dual-layer verification. A further 319 views were generated and scored in a full execution run (2{,}306 API calls, 9.41M tokens), with 319/319 truth-record anchor hits confirmed. Instrument calibration proceeded through three bounded gate rounds that moved merged format validity from $37.3$\% to $87.0$\%, with two DeepSeek generations eliminated ($21.9$\% and $18.8$\% valid rates) and seven channels excluded from the final design.

The partial fusion-preparation dry-run on the new cross-family panel shows encouraging signs: 2{,}181 of 2{,}744 main-layer units ($79.5$\%) have at least one valid vote, the covariate RE-LCA on this partial matrix yields $\hat\sigma=0.766$ (compared to $1.623$ on the legacy same-family panel), and per-unit posterior entropy drops dramatically (median $0.186$ vs.\ $0.981$ on the legacy panel). The cross-family panel carries substantially more per-unit information than the same-family panel it replaces---a direct consequence of breaking the family-level correlation that produced the 1.4-effective-vote finding.


==> sections_original/results_shell.tex <==
% Result-section shells. Every number in this section is a registered placeholder
% (see PLACEHOLDERS.md); prose frames are written to survive any branch of the
% preregistered interpretation grid.
\section{Reference Layer and Endpoints (Pending Phases 2--6)}
\label{sec:results-pending}

% Role: claim-first shells. Section compiles now; numbers arrive from the pipeline.
This section is scaffolded for the pending pipeline outputs. Its subsections mirror the experiment stages; every numeric slot is a registered placeholder keyed to its producing stage and fill window, and the interpretive frames quote the preregistered branches of Section~\ref{sec:grid} so that no post-hoc vocabulary can appear.

\subsection{Anchor blocks: judge accuracy on constructed truth (Phase 2)}
\label{sec:results-anchors}
Anchor blocks deliver per-judge, per-perturbation-class sensitivity and specificity with stratified gate checks: \PH{PHASE2-SE-SP} (point estimates and lower bounds per class), with demoted classes listed at \PH{PHASE2-DEMOTED-CLASSES} and injection blind-detectability at \PH{ANCHOR-HIDDENNESS}. Reporting follows the STARD 2015 flow structure with a QUADAS-2 four-domain self-appraisal (Section~\ref{sec:perturbations}, Appendix~\ref{app:quadas}); the construction premises of Section~\ref{sec:perturbations} are reported as audit outcomes rather than assumed---residual-quote-scan and residual-density pass rates, contradiction-screen outcomes, and out-of-window invariant checks per class: \PH{ANCHOR-PREMISE-AUDIT}. The Beta-prior equivalent sample sizes and transfer factor used downstream are registered at \PH{BETA-PRIOR-PARAMS}. Frame: classes failing the stratified gate are disclosed, not silently retained; anchor coverage matrices are public.

\subsection{Reference construction on contract-v2 votes (Phase 3)}
\label{sec:results-reference}
The fused reference reports: four-state composition over the main tier \PH{REF-COMPOSITION} (extension tier \PH{REF-COMPOSITION-EXT}); reference-level unsupported prevalence \PH{REF-PREVALENCE-CI} (participant-clustered interval; title-line precision row selected by realized $\hat p$ per Section~\ref{sec:precision}); hold-out calibration of the covariate latent-class model \PH{HOLDOUT-CAL}; entropy-calibration curve intercept/slope/ECE \PH{ENTROPY-CAL} with the back-solved unresolved threshold \PH{UNRESOLVED-THRESH}; the human-anchored overlap gate (corrected consensus vs.\ plurality, joint $\kappa$ difference) \PH{AAAI-OVERLAP-KAPPA}; and the formal four-state MTMM \PH{MTMM2-CONV}/\PH{MTMM2-DISC} with ratio \PH{MTMM2-RATIO}. Frame: if the overlap gate fails, the fusion layer downgrades and all downstream text says model-consensus reference regardless of audit.

\subsection{Reference validation: calibrated construction vs.\ simple aggregation (Phases 2--3, completed at 6)}
\label{sec:results-refvalidation}
The decisive reference-quality evidence is a head-to-head comparison of the calibration scheme against simple aggregation on \emph{identical inputs}, at \emph{matched cost}, over \emph{identical coverage}: \PH{REF-VALIDATION-TABLE}. Three arms consume the same judge votes: (a)~the calibrated scheme (MFRM corrected consensus fused with the anchor-prior RE-LCA and the unresolved threshold); (b)~plurality vote; (c)~a vote-averaging baseline (per-judge confidence mean with a fixed cut). Metrics: confident-error rate on anchor blocks---assignments made above the confidence threshold that are wrong against constructed truth---\PH{REFVAL-CONF-ERR}; agreement on human audit samples---the deferred random-quota and entropy-stratified adjudications of Section~\ref{sec:results-audit}---\PH{REFVAL-AUDIT-AGREE}; and coverage with unresolved rate over the main tier \PH{REFVAL-COVERAGE-UNRES}. Timing: computed after the Phase-3 votes and the Phase-2 fix-and-resend close out, before the reference freeze (the comparison uses panel votes and anchor truth only, so the anti-circularity firewalls of Section~\ref{sec:firewall} are respected); the audit-agreement column completes with Phase 6. Frame: this table, not internal-fit statistics, is the primary evidence that the calibrated construction earns its machinery; if a simple-aggregation arm matches it on anchor confident-error and audit agreement at equal coverage and unresolved rate, the claim vocabulary downgrades regardless of fit numbers. The design is registered as Amendment A2 to the frozen preregistration; the full specification ships with the release package.

\subsection{Endpoints (Phases 4--5)}
\label{sec:results-endpoints}
The model-conditional unsupported-correct rates enter the preregistered main table: \PH{MAINTABLE-J} and companions \PH{MAINTABLE-UD}, \PH{MAINTABLE-ABSTAIN}, \PH{MAINTABLE-FAIL}, \PH{MAINTABLE-COST}, with the primary tier contrast \PH{TIER-DIFF-CI} and sensitivity bounds \PH{UCR-LOWER}--\PH{UCR-UPPER}. Every UCR report in this paper appears as the fixed three-part set of Section~\ref{sec:estimand-udrn}---resolved-sample rate, unresolved share among hits, unresolved-treatment sensitivity---with the error-bounded skeleton of Section~\ref{sec:results-ucr}. Baselines (adapted sufficient-context autorater, ConText on EDAIC-only with disclosed Chinese-adaptation limits, templated NLI) report at \PH{BASELINES-TABLE}; perturbation paired contrasts $\tau$ per class at \PH{TAU-PERTURB}. Frame: the interpretation-grid branch realized by \PH{GRID-BRANCH} is quoted verbatim from Section~\ref{sec:grid}, always with its rival-explanation row (Table~\ref{tab:gridrivals}); no leaderboard titles under any branch.

\subsection{The UCR table: fixed trio with error bounds (Phase 5)}
\label{sec:results-ucr}
The unsupported-correct rate reports as a table, not a point estimate (Table~\ref{tab:ucrshell}). Participant-clustered bootstrap intervals bound every row; the magnitude check against reference error and the composition disclosure travel with the point estimates so that no UCR number is printed without its error context. If the magnitude check finds the observed rate comparable to the attribution-arm reference error rate, the realized grid branch is quoted with the cautious convergence caveat attached (Section~\ref{sec:estimand-udrn}); model-level contrasts are printed only next to their hit-sample composition disclosure.

\begin{table}[!htbp]
\centering\small
\caption{\textbf{UCR main-table skeleton (Phase 5).} Every row carries participant-clustered 95\% intervals; U/D split per the preregistration; the magnitude row lands with Phase 6.}
\label{tab:ucrshell}
\begin{tabularx}{\linewidth}{@{}l>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X@{}}
\toprule
Quantity & Definition & Slot (fill window) \\
\midrule
UCR, resolved sample & $(U+D)/(N-R)$ per tier $\times$ method arm, cluster-bootstrap 95\% CI; label-hit caliber $(U+D)/(C-R)$ alongside & \PH{UCR-MAINTABLE} (P5) \\
Unresolved share among hits & $R/C$ per tier $\times$ method arm & \PH{UCR-HIT-UNRESOLVED} (P5) \\
Unresolved-treatment sensitivity & registered bounds $[(U+D)/N,\,(U+D+R)/N]$ per row & \PH{UCR-SENSITIVITY} (P5) \\
Hit-sample composition & source $\times$ dimension $\times$ base-rate composition of each model's label-hit sample & \PH{UCR-COMPOSITION} (P5) \\
Magnitude check vs.\ reference error & observed UCR against $P(\text{reference wrong}\mid\text{judged unsupported})$ and the audit agreement bound & \PH{UCR-REFERR-COMPARE} (P6) \\
\bottomrule
\end{tabularx}
\end{table}

\subsection{Signal-detection decomposition of the main table (Phase 5)}
\label{sec:results-sdt}
The preregistered signal-detection layer of the five-pillar metrology closes here: model answers crossed with reference states yield hit and false-alarm rates per tier and method arm, summarized as $d'$ and area $A_z$ under the frozen mapping---abstentions are neither hits nor misses and are reported as their own arm-specific rate; hit and false-alarm cells receive the log-linear $+0.5$ correction before transformation; saturated arms (all-hit or all-false-alarm cells) are reported as non-estimable rather than imputed. Deliverables: the decomposition table \PH{SDT-DPRIME-TABLE} with tier-level $A_z$ contrasts \PH{SDT-AZ-TIER}, saturated-arm disclosure \PH{SDT-SATURATED-ARMS}, and the criterion-bias summary (the tendency to answer despite insufficient support) \PH{SDT-CRITERION-BIAS}. Frame: the SDT quantities are descriptive companions to the U/D/R/N estimands, never replacements; the $(U+D)/(N-R)$ family of Section~\ref{sec:estimand-udrn} governs all claims, and in an abstention-heavy paradigm $d'$ and $A_z$ are read as conditional-on-answer descriptive measures, not calibrated error probabilities.

\subsection{Attribution and terminal audit (Phases 4 and 6)}
\label{sec:results-audit}
The discordant attribution arm reports $P(\text{reference wrong}\mid\text{judged unsupported})=$ \PH{P-REF-ERR} (Wilson interval, participant-clustered; cannot-adjudicate bounds at \PH{P-REF-ERR-BOUNDS}). The random-quota audit arm reports per-source agreement \PH{AUDIT-PDCH} (PDCH) and \PH{AUDIT-EDAIC} (EDAIC), pooled \PH{AUDIT-RANDOM-ARM}, triggering claim tier \PH{AUDIT-CLAIM} by interval lower bound. Both terminal-audit arms additionally report an \emph{entropy stratification} (Amendment A1 to the frozen preregistration): audit agreement and reference-error rates are broken out for low-entropy high-consensus cells versus high-entropy cells, because a reference that is \emph{consistently} wrong at high consensus is invisible to discordant-only sampling---the discordant attribution arm already oversamples disagreement strata and here serves as the high-entropy stratum's counterpart: \PH{AUDIT-ENTROPY-STRATA}. Free-text adjudicator feedback is tabulated qualitatively at \PH{AUDIT-QUAL}. Frame: attribution informs interpretation only; the primary estimand is never adjusted; realized claim vocabulary follows the ladder of Section~\ref{sec:audit-ladder} exactly.

\subsection{Cost accounting}
\label{sec:results-cost}
Token-metered cost tables with matched budgets: reference panel \PH{COST-REFERENCE}, endpoint runs \PH{COST-ENDPOINTS}, against the preregistered pricing sheet with $<10\%$ deviation gate \PH{BUDGET-MATCH}.


==> teaser.tex <==
% Schematic dialogue and stipulated outputs; no patient excerpt or new result.
\begin{figure}[!ht]
\centering
\includegraphics[width=\linewidth]{figures/dataset_architecture.pdf}
\caption{\textbf{EviDial: from dialogue to traceable evidence.}
\textbf{(a)} An illustrative interview and native sleep label.
\textbf{(b)} The schematic map binds a denial to the patient and target window; blank cells do not denote negative symptoms.
\textbf{(c)} Removing that denial leaves the stipulated correct prediction unsupported.
The footer describes the legacy model annotation layer. Human component judgments are analyzed separately; task-aligned reference adjudication remains incomplete.}
\label{fig:architecture}\label{fig:teaser}\label{fig:model}
\end{figure}

